Supervised Laplacian embedding: bridging dimensionality reduction and sufficient dimension reduction

Dimensionality reduction in machine learning research has largely developed in isolation from sufficient dimension reduction in the statistical literature. In this paper, we first develop a new supervised Laplacian embedding method that addresses issues such as inappropriate normalization in existing approaches. We then develop statistical theory for the effectiveness of the proposed method, based on a novel, rigorous definition of an appropriate similarity measure that is also central to the framework of Laplacian embedding. Finally, we uncover the intrinsic connection between the proposed method and popular sufficient dimension reduction methods, thereby bridging the gap between machine learning research on dimensionality reduction and statistical research on sufficient dimension reduction for the first time in the literature. This connection benefits both communities in multiple ways: by bringing theoretical rigour to dimensionality reduction, by providing an algorithmic perspective on sufficient dimension reduction, and by generating new methods drawing on each other's literature. An example of the latter, called second-order supervised Laplacian embedding, is discussed in detail. Numerical studies are presented at the end.

==> macros1.tex <==
\RequirePackage{amsthm,amsmath,amsfonts,amssymb}
%\RequirePackage[numbers]{natbib}
%\RequirePackage[authoryear]{natbib}%% uncomment this for author-year citations
%\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
%\RequirePackage{graphicx}
\usepackage{latexsym, amsbsy, amssymb,amsmath,epsfig}
\usepackage{epsfig}
\usepackage{amsmath}
%\setlength{\textheight}{8.04in}
%\setlength{\textwidth}{5.43in}
%\setlength{\topmargin}{.16in}
%\setlength{\topmargin}{.9in}
%\setlength{\headheight}{0cm}
%\setlength{\oddsidemargin}{.545in}
%\setlength{\evensidemargin}{.55in}
%\renewcommand{\baselinestretch}{1.24}
%\renewcommand{\baselinestretch}{1.060}

%\setlength{\textheight}{8.04in}
%\setlength{\textwidth}{5.43in}
%\setlength{\topmargin}{.16in}
%\setlength{\topmargin}{.9in}
%\setlength{\headheight}{0cm}
%\setlength{\oddsidemargin}{.545in}
%\setlength{\evensidemargin}{.55in}
%\renewcommand{\baselinestretch}{1.24}
%




%\newtheorem{proposition}{{\bf Proposition}}
%\newtheorem{lemma}{{\bf Lemma}}
%\newtheorem{claim}{{\bf Claim}}
%\newtheorem{corollary}{{\bf Corollary}}
%\newtheorem{assumption}{{\bf Assumption}}
%\newtheorem{definition}{{\bf Definition}}
%\newtheorem{theorem}{{\bf Theorem}}
%\newtheorem{conjecture}{{\bf Conjecture}}

%\newtheorem{theorem}{{\bf Theorem}}
%\newtheorem{example}{{\bf Example}}
%\newtheorem{problem}{{\bf Problem}}
%\newtheorem{example}{{\bf Example}}
\newcounter{bean}
\def\=
{\hspace{-6pt}&=&\hspace{-6pt}}
\def\vec
{\mathrm{vec}}
\def\blb
{ \left\{
\begin{array}{c}
\vspace{8pt}
\end{array}
\right. \hspace{-8pt} }
\def\Zh
{\widehat{Z}}
\def\brb
{ \hspace{-8pt} \left.
\begin{array}{c}
\vspace{8pt}
\end{array}
\right\} }
%\newcommand{\real}[1]{\mathrm{I \! R} \mathit{^{#1}}}
%\newcommand{\real}[1]{{\mathbb R} \mathit{^{#1}}}
\newcommand{\realpl}[1]{\mathrm{I \! R} \mathit{_{+}^{#1}}}
\newcommand{\indep}{\;\, \rule[0em]{.03em}{.67em} \hspace{-.25em}
\rule[0em]{.65em}{.03em} \hspace{-.25em}
\rule[0em]{.03em}{.67em}\;\,}
\newcommand{\gvn}{\, \rule[0em]{.03em}{.67em} \,}
\newcommand{\sgvn}{\, \rule[0em]{.03em}{.44em} \,}
\newcommand{\ssgvn}{\, \rule[0em]{.03em}{.33em} \,}
\def\bdot{{{\raisebox{1pt}{\mbox{{\Large$.$}}}}}}
\newcommand{\supW}{^{^{(W)}}}
%\newcommand{\nsupseteq}{\not\supseteq}
\newcommand{\E}{\mathrm{E}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
%\newcommand{\spn}{\mathrm{Span}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\vecc}{\mbox{vec}}
\newcommand{\Ind}{\mbox{Ind}}
\newcommand{\drs}{{\sc drs}}
\newcommand{\cs}{{\sc cs}}
\newcommand{\cms}{{\sc cms}}
\newcommand{\pcs}{{\sc cps}}
\newcommand{\cpms}{{\sc cpms}}
\newcommand{\avp}{{\sc avp}}
\newcommand{\spc}{{\mathcal S}}
\newcommand{\lspc}{{\mathcal S}}
\newcommand{\vspc}{{\mathcal S}}
\newcommand{\uspc}{{\mathcal S}}
%\newcommand{\tyw}{\tilde{Y}_{w}}
%\newcommand{\lbm}{L}
\newcommand{\mols}{{\mathrm{ols}}}
\newcommand{\ols}{{\sc ols}}
\newcommand{\save}{{\sc save}}
\newcommand{\sir}{{\sc sir}}
\newcommand{\PHD}{{\sc PHD}}

\newcommand{\lv}{\mathrm{LV}}
\newcommand{\iv}{\mathrm{IV}}
\newcommand{\sz}{\mathrm{S}}
\newcommand{\fte}{\mathrm{FTE}}
\newcommand{\typ}{\mathrm{Typ}}
\newcommand{\wst}{\mathrm{Wst}}

%Bold Face symbols


\newcommand{\A}{{\mathbf A}}
\newcommand{\ba}{{\mathbf a}}
\newcommand{\B}{{\mathbf B}}
\newcommand{\bb}{{\mathbf b}}
\newcommand{\C}{{\mathbf C}}
\newcommand{\ia}{\theta}

\newcommand{\D}{{\mathbf D}}
\newcommand{\F}{{\mathbf F}}
\newcommand{\bg}{{\mathbf g}}
\newcommand{\h}{{\mathbf h}}
\newcommand{\bH}{{\mathbf H}}
\newcommand{\I}{{\mathbf I}}
\newcommand{\bell}{{\mathbf \ell}}
\newcommand{\M}{{\mathbf M}}
%\newcommand{\bm}{{\mathbf m}}
\newcommand{\Pb}{{\mathbf P}}
\newcommand{\Q}{{\mathbf Q}}
\newcommand{\bs}{{\mathbf s}}
\newcommand{\bt}{{\mathbf t}}
\newcommand{\U}{{\mathbf U}}
\newcommand{\bu}{{\mathbf u}}
\newcommand{\V}{{\mathbf V}}
\newcommand{\bv}{{\mathbf v}}
\newcommand{\X}{{\mathbf X}}
\newcommand{\bx}{{\mathbf x}}
\newcommand{\Z}{{\mathbf Z}}
\newcommand{\bz}{{\mathbf z}}
%
\newcommand{\1}{{\mathbf 1}}
\newcommand{\0}{{\mathbf 0}}

%Greek Bold Face symbols

\newcommand{\greekbold}[1]{\mbox{\boldmath $#1$}}
%
\newcommand{\alphabf}{\greekbold{\alpha}}
\newcommand{\betabf}{\greekbold{\beta}}
\newcommand{\rhobf}{\greekbold{\rho}}
\newcommand{\Gammabf}{\greekbold{\Gamma}}
\newcommand{\gammabf}{\greekbold{\gamma}}
\newcommand{\Deltabf}{\greekbold{\Delta}}
\newcommand{\deltabf}{\greekbold{\delta}}
\newcommand{\etabf}{\greekbold{\eta}}
\newcommand{\xibf}{\greekbold{\xi}}
\newcommand{\lambdabf}{\greekbold{\lambda}}
\newcommand{\mubf}{\greekbold{\mu}}
\newcommand{\Kappabf}{\greekbold{\Kappa}}
\newcommand{\Omegabf}{\greekbold{\Omega}}
\newcommand{\Phibf}{\greekbold{\Phi}}
\newcommand{\Psibf}{\greekbold{\Psi}}
\newcommand{\psibf}{\greekbold{\psi}}
\newcommand{\Sigmabf}{\greekbold{\Sigma}}
\newcommand{\sigmabf}{\greekbold{\sigma}}
\newcommand{\Thetabf}{\greekbold{\Theta}}
\newcommand{\thetabf}{\greekbold{\theta}}
\def\ker
{\mbox{ker}}
\def\lealign
{\hspace{-6pt}& \le &\hspace{-6pt}}
\def\gealign
{\hspace{-6pt}& \ge &\hspace{-6pt}}
%Greek Bold for subscripts

\newcommand{\gammabfs}{\greekbold{{\scriptstyle \gamma}}}
\newcommand{\Deltabfs}{\greekbold{{\scriptstyle \Delta}}}



% Cfig puts a figure of specified size centered on the current line.
%\newcommand{\Cfig}[2]{\centerline{\fbox{\psfig{figure=#1.eps,width=#2in}}}}
\newcommand{\Cfig}[2]{\centerline{\psfig{figure=#1.eps,width=#2in}}}
% Dfig puts a figure of specified size at the place indicated.
%\newcommand{\Dfig}[2]{\fbox{\psfig{figure=#1.eps,width=#2in}}}
\newcommand{\Dfig}[2]{\psfig{figure=#1.eps,width=#2in}}

\newenvironment{Efigs}[4]
         {\begin{figure}[#4]
                 \par
                 \Cfig{#1}{#3}
                \par
                  \caption{#2}
            \label{#1}
    \end{figure}}{}

\newenvironment{Efig}[2]{\Efigs{#1}{#2}{4}{p}}{}

\newenvironment{Etwofigs}[5]
   { %\vspace{.2in}
        \begin{figure} [t]
          \begin{center}
          \begin{tabular}{cc}
              \Dfig{#1}{2.0} & \Dfig{#3}{2.0} \\
             \footnotesize a. #2 & \footnotesize b. #4
             \normalsize
          \end{tabular}
          \caption{#5}
          \label{#1}\label{#3}
          \end{center}
        \end{figure}
 %  \vspace{.2in}
  }{}
\newenvironment{Ectwofigs}[5]
   { \vspace*{-1in}
        \begin{figure} [ht]
          \begin{center}
          \begin{tabular}{c}
              \Dfig{#1}{3.7} \\
             \footnotesize a. #2 \\
          \Dfig{#3}{3.7} \\
          \footnotesize b. #4
             \normalsize
          \end{tabular}
          \caption{#5}
          \label{#1}\label{#3}
          \end{center}
        \end{figure}
 %  \vspace{.2in}
  }{}
\newenvironment{Efourfigs}[9]
   { %\vspace{.2in}
        \begin{figure} [p]
          \begin{center}
          \begin{tabular}{cc}
               \Dfig{#1}{2.75} & \Dfig{#3}{2.75} \\
             \footnotesize a. #2 & \footnotesize b. #4 \\
             \normalsize
               \Dfig{#5}{2.75} & \Dfig{#7}{2.75} \\
             \footnotesize c. #6 & \footnotesize d. #8
             \normalsize
          \end{tabular}
          \label{#1}\label{#3}\label{#5}\label{#7}
          \caption{#9}
          \end{center}
        \end{figure}
 %  \vspace{.2in}
  }{}

\def\and
{\mbox{and}}
\def\argmin
{\mathrm{argmin}}
\def\cov
{\mathrm{cov}}
\def\ran
{\mathrm{ran}}
%\def\proof
%{\noindent
%{\sc Proof.   }
%}
\def\speculation
{\noindent
{\sc Speculation.   }
}
\def\eop
{\hfill $\Box$ \vspace{.1in}
}
%\def\eop
%{\hfill $\Box$ \\
%
%\vspace{-.2in}}
\def\blp
{ \left(
\begin{array}{l}
\vspace{5pt}
\end{array}
\right.
\hspace{-13pt}
}
\def\brp
{\hspace{-13pt}
\left.
\begin{array}{l}
\vspace{5pt}
\end{array}
\right)}
\def\msave
{M_{\mathrm{SAVE}}}
\def\msir
{M_{\mathrm{SIR}}}
\def\trace
{\mathrm{tr}}

